Petri Nets with Parameterised Data: Modelling and Verification (Extended Version)

During the last decade, various approaches have been put forward to integrate business processes with different types of data. Each of such approaches reflects specific demands in the whole process-data integration spectrum. One particular important point is the capability of these approaches to flexibly accommodate processes with multiple cases that need to co-evolve. In this work, we introduce and study an extension of coloured Petri nets, called catalog-nets, providing two key features to capture this type of processes. On the one hand, net transitions are equipped with guards that simultaneously inspect the content of tokens and query facts stored in a read-only, persistent database. On the other hand, such transitions can inject data into tokens by extracting relevant values from the database or by generating genuinely fresh ones. We systematically encode catalog-nets into one of the reference frameworks for the (parameterised) verification of data and processes. We show that fresh-value injection is a particularly complex feature to handle, and discuss strategies to tame it. Finally, we discuss how catalog nets relate to well-known formalisms in this area.

==> 2-dbnet_old.tex <==
\section{The \dbnet Formal Model}




In this section, we briefly present the key concepts and notions used for defining \dbnets. Conceptually, a \dbnet is composed of three layers (cf. Figure~\ref{fig:dbnets})
\begin{inparaenum}[1)]
\item \emph{persistence layer}, capturing a full-fledged relational database with constraints,
and used to store background data, and data that are persistent across cases;
\item \emph{control layer}, employing a variant of CPNs to capture the process control-flow,
case data, and possibly the resources involved in the process execution;
\item \emph{data logic layer}, interconnecting in the persistence and the control layer.
\end{inparaenum}
We next formalize the framework layer by layer and define its execution semantics. 

\subsection{Syntax}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%			PERSISTENCE LAYER				%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\smallskip\noindent
\textbf{Persistence layer.} A \emph{type domain} $\types$ is a finite set of pairwise disjoint \emph{data types} $\type=\tup{\dom_\type,\sigp_\type,\Sigma_\type}$, where a set $\dom_\type$ is a \emph{value domain}, $\sigp_\type$ is a finite set of \emph{predicate  symbols} and $\Sigma_\type$ is the signature interpretation, i.e., a function associating each predicate symbol $S$ of arity $n$, denoted as $S/n$, to an $n$-ary relation $\Sigma(S)\subseteq \dom_\type^n$.
Examples of data types are:
\begin{inparaenum}[\it (i)]
\item $\typename{string} = \tup{\strings,\set{=_s},\Sigma_s}$, strings with the equality predicate;
%, where $s_1 = s_2$ if and only if $s_1$ and $s_2$ are the same string;
\item $\typename{real} = \tup{\reals,\set{=_r,<_r},\Sigma_r}$, reals with the usual comparison operators; 
\item $\typename{int} = \tup{\ints,\set{=_{int},<_{int},succ},\Sigma_{int}}$, integers with the usual comparison operators, as well as the successor predicate.
\end{inparaenum}
\todo[inline]{Here, one could compare "our" datatypes with color types in CPN}
\todo[inline]{How can we represent type-specific operations in MCMT? Through additional axioms added to every particular model? Will it be then smth similar to the way it's done for algebraic Petri nets (via Maude)?}
We call $R(a_1:\type_1,\ldots,a_n:\type_n)$ a \emph{$\types$-typed relation schema}, where $R$ is a relation name and $a_i:\type_i$ indicates the $i$-th attribute of $R$ together with its data type. When no ambiguity arises, we shall omit explicitly mentioning relation attributes and/or their data types. 
A \emph{$\types$-typed database schema} $\schema_\types$ is a finite set of $\types$-typed relation schemas.
A \emph{$\types$-typed database instance $\I$ over $\schema_\types$} is a finite set of facts of the form $R(\cname{o_1},\ldots,\cname{o_n})$, where 
$R\in \schema$ and $\cname{o_i}\in \dom_{\type_i}$, for $i \in \set{1,\ldots,n}$.
%Given a type $\type \in \types$, the \emph{$\type$-active domain of $\I$}, is the set of $\adom[\type]{\I}=\set{\cname{o} \in \dom_\type\mid \cname{o} \text{ occurs in }\I}$. 

Given $\types$, we fix a countably infinite set $\varset$ of typed variables with a \emph{variable typing function} $\vartype: \varset \rightarrow \types$. Note that such function can be suitably extended to account for sets, tuples and multisets of variables as well as constants. 
As the query language we opt for the union of conjunctive queries with inequalities and atomic negations that can be specified in terms of first-order (FO) logic extended with types. 
A \emph{(well-typed) conjunctive query (CQ)} $Q$ over $\schema_\types$ is a formula of the form: 
\[Q::=\varphi~\mid~R(x_1,\ldots,x_n)~\mid~\neg R(x_1,\ldots,x_n)~\mid~Q \land Q~\mid~\exists x.Q,\text{ where}\] 
\begin{inparaenum}[\it(i)]
\item $R(\type_1,\ldots,\type_n)\in\schema$, $x\in\varset$ and each $x_i$ is either a variable of type $\type_i$ or a constant from $\dom_{\type_i}$;
\item $\varphi::=S(y_1,\ldots,y_m)~\mid~\neg\varphi~\mid~\varphi\land\varphi$ is a \emph{condition} s.t. $S\in\sigp_\type$ and $y_i$ is either a variable of type $\type$ or a constant from $\dom_{\type}$.
\end{inparaenum}
We use $\cqd$ to denote a set of all such conjunctive queries and $\free{Q}$ to denote a set of all free variables (i.e., those not occurring in the scope of quantifiers) of query $Q$. 
%The definition of the $\free$ function can be naturally extended to sets of queries. 
We also use $\conds$ to denote a set of all possible conditions and $\varsin{Q}$ to denote the set of all variables in $Q$.
A \emph{boolean query} is a query without free variables. With $\ucqd$ we shall denote a set off all \emph{unions of conjunctive queries} over $\schema_\types$, where each query $Q\in\ucqd$ is defined as $Q=\bigwedge_{i=1}^n Q_i$, s.t. every $Q_i\in\cqd$. 
Finally, given a query $Q$ such that $\free{Q} = \set{x_1, \ldots , x_n}$, we employ notation $\query{q}{x_1,\ldots,x_n}{Q}$ to emphasize the free variables of $Q$, and to fix a natural ordering over them.
 



A \emph{substitution} for a set $X = \set{x_1,\ldots,x_n}$ of typed variables,
is a function $\subst: X \rightarrow \dom_\types$, such that
$\subst(x) \in \dom_{\vartype(x)}$, for every $x \in X$. An empty substitution is denoted as $\tup{}$.  A \emph{substitution
 $\subst$ for a query $Q$}, denoted as $Q\subst$, is a substitution for variables in $\free{Q}$. 
%We denote by $Q\subst$ the boolean query obtained from $Q$ by replacing
%each occurrence of a free variable $x \in \free{Q}$ with the value $\subst(x)$.
%
An \emph{answer to a query $Q$} in an instance $\I$ is a set of substitutions $\ans(Q,\I) = \{ \subst: \free{Q} \rightarrow \adom{\I} \mid
\qent{\I}{\subst}{Q}\}$, where $\adom{\I}$ is the set of all constants occurring in $\I$, called an \emph{active domain},  and $\models$ denotes standard FO entailment. 
%Given a $\types$-typed database schema $\schema$, a $\types$-typed instance
%$\I$ over $\schema$, and a \fod query $Q$ over $\schema$, the set of
%\emph{answers} to $Q$ in $\I$ is defined as the set
%$\ans(Q,\I) = \{ \subst: \free{Q} \rightarrow \adom[\types]{\I} \mid
%\qent{\I}{\subst}{Q}\}$ of substitutions for $Q$, where $\models$ denotes
%standard FO entailment (i.e., we use \emph{active-domain semantics}).
%%%
When $Q$ is boolean, we shall write $\ans(Q,\I) \equiv \true$ if $\ans(Q,\I)=\set{\tup{}}$ , and $\ans(Q,\I) \equiv \false$ if $\ans(Q,\I) = \emptyset$.
Boolean queries are also used to express \emph{constraints} over $\schema$.  
%We introduce explicitly two common types of constraints: given relations $R/n$ and $S/m$,
%and two index-sets $N$ and $M$ such that $1\leq i\leq n$ for every $i\in N$,
%and $1\leq j\leq m$ for every $j \in M$, we fix the following notation:
%\begin{inparaenum}[\it (i)]
%\item  $\PKindex{R}{N}$ expresses that the projection
%  $\projindex{R}{N}$ of $R$ on $N$ is a primary key for $R$;
%\item $\FKindex{R}{N}{S}{M}$ expresses that the projection $\projindex{R}{N}$ of $R$ on
%  $N$ refers the projection $\projindex{S}{M}$ of $S$ on $M$, which has to be a key
%  for $S$.
%\end{inparaenum}
%Both kinds of constraints are obviously expressible as suitable queries~\cite{AbHV95}.

%
%Boolean queries are also used to express \emph{constraints} over $\schema$,
%required to hold over each database instance, i.e., a database instance $\I$
%satisfies a constraint $\Phi$ if $\ans(\Phi,\I) \equiv \true$.  
\begin{definition}
A $\types$-typed \emph{persistence layer} $\pers$ is a pair $(\schema,\cset)$ where:
\begin{inparaenum}[\it (i)]
\item $\schema$ is a $\types$-typed database schema;
\item $\cset$ is a finite set $\{\Phi_1,...,\Phi_k\}$ of boolean \fod queries over $\schema$, modelling \emph{constraints over $\schema$}.
\end{inparaenum}
\end{definition}
We say that a $\types$-typed database instance $\I$ \emph{complies with} $\pers$, if $\I$ is defined over $\schema$ and satisfies all constraints in $\cset$.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%			DATA LOGIC LAYER				%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\medskip
\noindent
\textbf{Data logic layer.} The data logic layer allows one to extract data from the database  using queries as well as to update the database by adding and deleting possibly multiple facts at once. 
%The data logic layer provides functionality for updating the database by adding and deleting possibly multiple facts at once. 
Such updates follow the \emph{transactional} semantics. That is, if a new database instance obtained after some update is still compliant with the persistence layer, the update is \emph{committed}; otherwise it is \emph{rolled back}. 
Such updates are realized in parametric atomic actions that consist of expressions with fact templates that, after being instantiated, will be added to and deleted from the database. 
A fact template of $R(\type_1,\ldots,\type_n)\in\schema$ over $\vec{p}$ is defined as $R(y_1,\ldots,y_n)$, s.t. every $y_i$ is either a constant or a variable from $\vec{p}$, both of type $\type_i$. 

%This approach is in line with how database management systems operate in practice.

A \emph{(parameterized) action} $\action(\vec{p})$ over a $\types$-typed persistence layer $(\schema,\cset)$ is a tuple $\tup{F^+,F^-}$, where:
\begin{inparaenum}[\it (i)]
	\item $\vec{p}$ is a tuple of pairwise distinct variables from $\varset$, denoting the \emph{action (formal) parameters};
	\item $F^+$ and $F^-$ respectively represent a finite set of $R$-fact templates for some $R\in\schema$ over $\vec{p}$ to be \emph{added} to and \emph{deleted} from the current database instance.
\end{inparaenum}
To access the different components of an action $\action$, we use a dot notation: 
%$\apar{\action} = \vec{p}$, 
$\aadd{\action}= F^+$, and $\adel{\action}=F^-$.


%Given an action $\action$ and a (parameter) substitution $\subst$ for $\apar{\action}$, we call \emph{action instance $\action\subst$} the (ground) action resulting by substituting parameters of $\action$ with corresponding values from $\subst$. Then, given a $\types$-typed database instance $\I$ compliant with $\types$, the \emph{application} of $\action\subst$ on $\I$, , written $\doact{\action\subst}{\I}$, is a database instance over $\schema$ obtained as $(\I\setminus F^-_{\action\subst})\cup F^+_{\action\subst}$, where:
%\begin{inparaenum}[\it (i)]
%\item $F^-_{\action\subst} = \bigcup_{R(\vec{y}) \in \adel{\action}} R(\vec{y})\subst$;
%\item $F^+_{\action\subst} = \bigcup_{R(\vec{y}) \in \aadd{\action}} R(\vec{y})\subst$.
%\end{inparaenum}
%If $\doact{\action\subst}{\I}$ complies with $\pers$, $\action\subst$ can be \emph{successfully applied} to $\I$. 
%Note that, in order to avoid situations in which the same fact is asserted to be added and deleted, we prioritize additions over deletions.

\begin{definition}
	Given a $\types$-typed persistence layer $\pers$, a \emph{$\types$-typed data logic layer over $\pers$} is a pair $(\queries,\actions)$, where:
	\begin{inparaenum}[\it (i)]
	\item $\queries$ is a finite set of \fod queries over $\pers$;
	\item $\actions$ is a finite set of actions over $\pers$.
	\end{inparaenum}
\end{definition}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%			CONTROL LAYER				%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Control layer.} The control layer employs a fragment of Coloured Petri net to capture the process control flow and a data logic to interact with an underlying persistence layer.
We fix some preliminary notions. We consider the standard notion of a \emph{multiset}. Given a set $A$,  the \emph{set of multisets} over $A$, written $\mult{A}$, is the set of mappings of the form $m:A\rightarrow \mathbb{N}$.
Given a multiset $S \in \mult{A}$ and an element $a \in A$, $S(a) \in \mathbb{N}$ denotes the number of times $a$ appears in $S$.  Given $a \in A$ and $n \in \mathbb{N}$, we write $a^n \in S$ if $S(a) = n$.  We also consider the usual operations on multisets. Given $S_1,S_2 \in \mult{A}$:
\begin{inparaenum}[\it (i)]
\item $S_1 \subseteq S_2$ (resp., $S_1 \subset S_2$) if $S_1(a) \leq S_2(a)$ (resp., $S_1(a) < S_2(a)$) for each $a \in A$;
\item $S_1 + S_2 = \set{a^n \mid a \in A \text{ and } n = S_1(a) + S_2(a)}$;
\item if $S_1 \subseteq S_2$, $S_2 - S_1 = \set{a^n \mid a \in A \text{ and } n = S_2(a) - S_1(a)}$;
\item given a number $k \in \mathbb{N}$, $k \cdot S_1 = \set{a^{kn} \mid a^n \in S_1}$.
\end{inparaenum}

%We also employ a usual notion of a net structure. A net structure is a tuple $N=(\places,\transitions,\flow)$ such that:
%\begin{inparaenum}[\it 1)]
%\item $P$ and $T$ are finite sets of places and transitions, s.t. $P\cap T=\emptyset$;
%\item $\flow\subseteq (\places\times\transitions)\cup(\transitions\times\places)$ is a flow relation.
%\end{inparaenum}
%Given a node $x\in \places\cup\transitions$, the set $\pre{x}=\set{y\mid (y,x)\in \flow}$ is the pre-set of $x$ and the set $\post{x}=\set{y\mid (x,y)\in\flow}$ is the post-set of $x$.

%We shall call \emph{inscription} a set of typed variables (and, possibly, values) and denote the set of all possible inscriptions over set $\mathcal{Y}$ as $\tuples{\mathcal{Y}}$, and the set of variables appearing inside an inscription $\omega \in \tuples{\mathcal{Y}}$ as $\varsin{\omega}$ (such notation naturally extends to sets and multisets of inscriptions).  
In the spirit of CPNs, the control layer assigns to each place a color type, which in turn combines one or more data types from $\types$. 
Contents of places can be referenced via \emph{inscriptions} -- tuples of variables and constants. We denote by $\Omega_A$ the set of all possible inscriptions over a set $A$ and, with slight abuse of notation, use $\varsin{\omega}$ to denote the set of variables of $\omega\in\Omega_A$.
%Formally, a \emph{$\types$-color} is $\type_1 \times \ldots \times \type_m$, where for each $i \in \set{1,\ldots,m}$, we have $\type_i \in \types$. We denote by $\colors$ the set of all possible $\types$-colors.
To account for fresh external inputs, we employ the well-known mechanism adopted in $\nu$-Petri nets~\cite{RVFE11} and introduce a countably infinite set $\nuvarset$ of $\types$-typed \emph{fresh variables}, where for every $\nu \in \nuvarset$, we have that $\dom_{\vartype(\nu)}$ is countably infinite (this is done to guarantee an unlimited supply of fresh values). Hereinafter, we fix a countably infinite set of $\types$-typed variable $\vars = \varset \cup \nuvarset$ as the disjoint union of ``normal" variables $\varset$ and fresh variables $\nuvarset$. 

\begin{definition}
A $\types$-typed \emph{control layer} over a data logic layer $\dl = \tup{\queries,\actions}$ is a tuple
$(\places,\transitions,\inflow,\outflow,\coloring,\quass,\guass,\aass)$, where:
\begin{compactenum}
%
%\item $(\places,\transitions,\flow)$ is a net structure;
\item $\places$ and $\transitions$ are finite sets of places and transitions, s.t. 
\begin{compactitem}
\item $P\cap T=\emptyset$ and
\item $\places = \cplaces \cup \vplaces$, where $\cplaces$ is a set control places and $\vplaces$ is a set of view places; 
\end{compactitem}
%
\item $\coloring: \places \rightarrow \powerset(\types)$ is a place typing function;
\item $\quass: \vplaces \rightarrow \ucqd$ is a query assignment function, s.t. $\vartype(\free{\quass(p)})=\coloring(p)$ for every $p\in\vplaces$;
%mapping each view place $p \in \vplaces$ with $\coloring(p) = \type_1\times\ldots\times\type_n$ to a query $Q(x_1,\ldots,x_n)$ from $\queries$, s.t. the color of $p$ component-wise matches with the types of the free variables in $Q$: for each $i \in \set{1,\ldots,n}$, we have $\type_i = \vartype(x_i)$.
%
\item $\inflow: \places \times \transitions \rightarrow \mult{\Omega_{\varset}}$ is an input flow, 
%assigning multisets of inscriptions to input arcs, 
s.t. $\vartype(\inflow(p,t))=\coloring(p)$ for every $(p,t)\in\places\times\transitions$;
\item $\outflow: \transitions \times \cplaces \rightarrow \mult{\tuples{\vars \cup \dom_\types}}$ is an output flow, s.t. $\vartype(\outflow(t,p))=\coloring(p)$ for every $(t,p)\in\transitions\times\places$;
%each of such inscriptions $\omega$ is compatible with each of its input places $p$, i.e., for every $i \in \set{1,\ldots,m}$, we have $\vartype(x_i) = \type_i$, where $\coloring(p) = \type_1 \times \ldots\times \type_m$.
%
\item $\guass:  \transitions \rightarrow \conds$ is a partial guard assignment function, s.t.  $\varsin{\guass(t)}\subseteq\invars{t}$ for every $t\in\transitions$, with $\invars{t}=\cup_{p\in\places}\varsin{\inflow(p,t)}$;
\item $\aass: \transitions \rightarrow \actions \times \tuples{\vars \cup \dom_\types}$ is a partial action assignment function, where $\aass(t)$ maps $t$ to an action $\action(p_1\ldots,p_m) \in \actions$ together with a (binding) inscription $\tup{y_1,\ldots,y_m}$, s.t.  $\vartype(y_i) = \vartype(z_i)$ if $y_i\in\vars$, or $y_i \in \dom_{\vartype(z_i)}$ if $y_i\in\dom_\types$, for each $i \in \set{1,\ldots,m}$. 
%\begin{compactitem}[$\bullet$]
%\item $\invars{t} = \set{x \in \varset \mid \text{there exists }p \in \places \text{ such that }x \in \varsin{\inflow(\tup{p,t})}}$ is the set of all variables occurring on input arc inscriptions of $t$;
%\item a $\types$-typed \emph{guard} from is a formula (or a quantifier- and relation-free \fod query) of the form $\varphi~::=~\true \mid S(\vec{y}) \mid \neg \varphi  \mid \varphi_1 \land \varphi_2$, where $S/n\in\sigp_\type$ and, for $\vec{y} = \tup{y_1,\ldots,y_n} \subseteq \varset$, we have that  $y_i$ is either a value $\cname{o} \in \dom_{\type}$, or a variable $x_i \in \varset$ with $\vartype(x_i) = \type$ ($i \in \set{1,\ldots,n}$);
%\item $\guards{\types}$ is the set of all possible $\types$-typed guards and, with a slight abuse of notation, $\varsin{\varphi}$ is the set of variables occurring in $\varphi$.
%\end{compactitem}
%

%
\end{compactenum}
%
\end{definition}

Here, view places allow the net to inspect parts of the database using queries. Graphically such places are represented as \resizebox{.35cm}{!}{\tikz{\node [circle,draw,very thick,minimum width=.6cm, minimum height=.6cm] at (0,0) {}; \dbicon{(0,0)}{.4cm}{.3cm}}} and are always connected to transitions with special read arcs. 
%We also make use of the usual Petri net notation of pre- and post-sets. Given a node $x\in \places\cup\transitions$, the set $\pre{x}=\set{y\mid (y,x)\in \flow}$ is the pre-set of $x$ and the set $\post{x}=\set{y\mid (x,y)\in\flow}$ is the post-set of $x$.

%According to the diagram in Figure~\ref{fig:dbnets}, the \dbnet control layer can be obtained on top of \nucpns by essentially adding three mechanisms that allow the net to interact with the underlying persistent storage:
%\begin{inparaenum}[\it (i)]
%\item view places, a;
%\item action binding, linking atomic actions and their parameters to transitions and their inscription variables;
%\item rollback transition-place arcs, enacted when the action application induced by a transition firing violates some database constraint, so as to explicitly account for ``error-handling''.
%\end{inparaenum}


\begin{definition}
A \emph{db-net} is a tuple $\tup{\types,\pers,\dl,\cl}$, where:
\begin{inparaenum}[\it (i)]
\item $\types$ is a type domain;
\item $\pers$ is a $\types$-typed persistence layer;
\item $\dl$ is a $\types$-typed data logic layer over $\pers$;
\item $\cl$ is a $\types$-typed control layer over $\dl$.
\end{inparaenum}
\end{definition}
%\todo[inline]{Do we need notions of $\outvars{t}$??}
%To properly manage variables occurring in the action assignment for $t$ (if any), and in its output arc inscriptions, we define a set of \emph{output variables} of $t$ as $\outvars{t} = \apar{\aass(t)} \cup \set{\varsin{\outflow(\tup{t,p})}\mid p\in\places}$.
%%  \[\outvars{t} = \begin{array}[t]{ll}
%%  	& \set{x \in \vars \mid \aass(t) \text{ is defined as } \tup{\alpha,\omega}, \text{ and } x \in \varsin{\omega}}\\  
%%  	\cup &
%% 	\set{x \in \vars \mid \text{there exists }p \in \places \text{ such that }x \in \varsin{\outflow(\tup{t,p})}}.
%%  	\end{array}  
%%    \]
%Using this notion we can obtain the \emph{external variables} of $t$ as $\outvars{t} \setminus \invars{t}$. 
%Each such variable $x$ is not bound by any input inscription, and can be either arbitrarily instantiated (if $x \in \varset$), or assigned to a fresh value (if $x \in \nuvarset$). Among such variables, we explicitly refer to the fresh variables attached to $t$ as $\freshvars{t} = \outvars{t} \cap \nuvarset$.


\subsection{Semantics}

The execution semantics of a \dbnet simultaneously accounts for the progression of a database instance compliant with the persistence layer of the net, and for the evolution of a marking over the control layer of the net. 
Thus, a to represent a state of the net we use a notion of a \emph{snapshot}. 
More specifically, a snapshot of a \emph{db-net} $\tup{\types,\pers,\dl,\cl}$ is a tuple $(\I,m)$, where:
\begin{compactitem}
\item $\I$ is a database instance compliant with $\pers$,
\item $m:\places\rightarrow \mult{\Omega_\types}$ is a marking function, s.t.  $m(p)\in\mult{\dom_{\coloring(p)}}$ for every $p\in\places$ and  $m(v)=\ans(\quass(v),\I)$ for every $v\in\vplaces$ ($m$ is \emph{aligned} to $\I$ via $\quass$).
\end{compactitem}

As customary for CPNs, the firing of a transition $t$ in a snapshot is defined w.r.t. a so-called \emph{binding} for $t$ defined as $\sigma : \varsin{t} \rightarrow \types$\footnote{Note that a definition of $\sigma$ can be naturally extended to multisets.}, where $\varsin{t}=\invars{t}\cup\outvars{t}$ with $\outvars{t}=\cup_{p\in\places}\varsin{\outflow(t,p)}\cup \varsin{\omega}$ and $\aass(t)=\tup{\action(\vec{p}),\omega}$.
A transition $t \in\transitions$ is \emph{enabled} in a snapshot $\tup{\I,m}$ iff there exists a binding $\sigma$ and the following conditions hold:
\begin{inparaenum}[\it (1)]
\item  $m(p) \geq \sigma(\inflow(p,t))$, for every $p\in\places$;
\item $\sigma(\guass(t))$ is true;
\item $\sigma(x)\not\in \adom{m}_{\vartype(x)} \cup \adom{\I}_{\vartype(x)}$, for
every $x\in\nuvarset \cap \outvars{t}$.
% ($\sigma$ assigns globally fresh values to fresh variables in the expressions attached to arcs outgoing from $t$).
\end{inparaenum}

When a transition $t$ is enabled, it may fire. Its firing with some binding has then a threefold effect. First, all tokens present in input places of $t$ that match inscriptions on corresponding arcs are consumed. Second, an action assigned to $t$ updates the current persistent storage instance. Third, tokens built after the inscriptions on output arcs are produced and put into target places.

\begin{definition}
Let $\tup{\types,\pers,\dl,\cl}$ be a \dbnet, $s=\tup{I,m}$ is its snapshot and $t\in\transitions$ is a transition enabled in $s$ with some binding $\sigma$. Then, $t$ may \emph{fire} producing a new snapshot $\tup{I',m'}$ such that:
\begin{compactitem}
\item $\I'=(\I\setminus F^-_{\action(\sigma(\vec{p}))})\cup F^+_{\action(\sigma(\vec{p}))}$, where 
\begin{inparaenum}[\it (i)]
\item $\aass(t)=\tup{\action(\vec{p}),\omega}$, 
\item $F^-_{\action(\sigma(\vec{p}))} = \bigcup_{R(\vec{y}) \in \adel{\action}} R(\vec{y})\sigma$,
\item $F^+_{\action(\sigma(\vec{p}))} = \bigcup_{R(\vec{y}) \in \aadd{\action}} R(\vec{y})\sigma$;
\end{inparaenum}
\item $m'(p)=m(p)-\sigma(\inflow(p,t))+\sigma(\outflow(t,p))$ for every $p\in\cplaces$.
\end{compactitem}
Note that a new state is generated only if $\I'$ is compliant with $\pers$. Otherwise, $\tup{I',m'}=\tup{I,m}$.
\end{definition}

\endinput
Given an action $\action$ and a (parameter) substitution $\subst$ for $\apar{\action}$, we call \emph{action instance $\action\subst$} the (ground) action resulting by substituting parameters of $\action$ with corresponding values from $\subst$. Then, given a $\types$-typed database instance $\I$ compliant with $\types$, the \emph{application} of $\action\subst$ on $\I$, , written $\doact{\action\subst}{\I}$, is a database instance over $\schema$ obtained as $(\I\setminus F^-_{\action\subst})\cup F^+_{\action\subst}$, where:
\begin{inparaenum}[\it (i)]
\item $F^-_{\action\subst} = \bigcup_{R(\vec{y}) \in \adel{\action}} R(\vec{y})\subst$;
\item $F^+_{\action\subst} = \bigcup_{R(\vec{y}) \in \aadd{\action}} R(\vec{y})\subst$.
\end{inparaenum}
If $\doact{\action\subst}{\I}$ complies with $\pers$, $\action\subst$ can be \emph{successfully applied} to $\I$. 
Note that, in order to avoid situations in which the same fact is asserted to be added and deleted, we prioritize additions over deletions.



\endinput
Due to space limitations, we refer to the definition of the formal semantics studied in~\cite{MonR17}. 
We thus assume that the execution semantics of both \nucpns and \dbnets can be captured with a possibly infinite-state labeled transition system (LTS) that accounts for all possible executions starting from their initial markings. 
While transitions in such LTSs model the effect of firing nets under given bindings, their state representations slightly differ. Namely, in the case of \nucpns we have markings (like, for example, in coloured Petri nets~\cite{JeK09}), while in the case of \dbnets one also has to take into account database states. 
W.l.o.g., we shall use $\tsys{M_0}{\cpn} = \tup{\M,M_0,\trans,L}$ to specify an LTS for a \nucpn $\cpn$ with initial marking $M_0$ and $\tsys{\istate}{\dbn} = \tup{\states,\istate,\trans,L}$ to specify an LTS for a \dbnet $\dbn$ with initial snapshot $\istate=\tup{\I_0,m_0}$, where $\I_0$ is the initial database instance and $m_0$ is the initial marking of the control layer.



==> 2-reponet_long.tex <==

\newcommand{\datatype}[1]{\texttt{#1}}

\section{The \clognet Formal Model}

%\todo[inline]{say that our model is $\nu$-CPNs extended with an ability to query read-only databases; derived framework is also a fragment of \dbnets}


In this section, we briefly present the key concepts and notions used for defining \clognets. Conceptually, a \clognet combines in one integrated model two key components. On the one hand, it accounts for a read-only persistent data storage, called \emph{catalog}, to account for read-only, parameterised data.
On the other hand, it includes a variant of a coloured Petri net, called \nucpn \cite{MonR19}, to represent the process backbone. In this net, each token carries a tuple of data objects, which can be seen, depending on the usage, as a carried payload or as a record of a relation stored in a place. Places of this net are typed and can be used to represent: 
\begin{inparaenum}[\it (i)]
\item states of (interrelated) case objects, 
\item read-write relations, 
\item read-only relations whose extension is fixed (and consequently not subject to parameterisation), 
\item resources. 
 \end{inparaenum}
As in \cite{MonR19}, the net employs the well-established notion of $\nu$-variables (first studied in the context of \nupns~\cite{RVFE11}) to inject fresh data (such as object identifiers). Differently from \cite{MonR19}, in \clognets transitions can have guards that inspect and retrieve data objects from the read-only, persistent storage, and compare them with the data carried by tokens.   


%
%Conceptually, a \clognet can be seen as a \nucpn~\cite{MonR19} enriched with a read-only persistent data storage called a catalog.
%
%For example, enriching tokens with names (of objects from some abstract domain) that can be only compared for equality and allowing a net to generate fresh ones along its run, leads to a formalism called \nupns~\cite{main_VelardoF08} for which only coverability, termination and boundedness are decidable. Using this Petri net class, it is possible to construct models that can be of great help for representing data-aware processes in which one may naively cast away the persistence storage, but at the same time preserve on the abstract level the data generation, migration and comparison.


%\begin{inparaenum}[1)]
%\item \emph{persistence layer}, capturing a full-fledged relational database with constraints,
%and used to store background data, and data that are persistent across cases;
%\item \emph{control layer}, employing a variant of CPNs to capture the process control-flow,
%case data, and possibly the resources involved in the process execution;
%\item \emph{data logic layer}, interconnecting in the persistence and the control layer.
%\end{inparaenum}
%We next formalize the framework layer by layer and define its execution semantics. 

%\todo[inline]{Introduce explicit primary key and foreign key relations to data objects. Explain then how these things are going to correspond to sorts.}

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%		DATA TYPES	      %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%


\smallskip\noindent
\textbf{Catalog.} 
We consider a \emph{type domain} $\types$ as a finite set of pairwise disjoint data types accounting for the different types of objects existing in the domain (such as orders, items, and trucks). Each type $\type \in \types$ comes with its own (possibly infinite) \emph{value domain} $\dom_\type$, and with an equality operator $=_\type$. When clear from the context we simplify the notation and simply use $=$ in place of $=_\type$.
%A \emph{type domain} $\types$ is a finite set of pairwise disjoint \emph{data types} $\type=\tup{\dom_\type,\sigp_\type,\Sigma_\type}$, where a set $\dom_\type$ is a \emph{value domain}, $\sigp_\type$ is a finite set of \emph{predicate  symbols} and $\Sigma_\type$ is the signature interpretation, i.e., a function associating each predicate symbol $S$ of arity $n$, denoted as $S/n$, to an $n$-ary relation $\Sigma(S)\subseteq \dom_\type^n$.
%Examples of data types are:
%\begin{inparaenum}[\it (i)]
%\item $\typename{string} = \tup{\strings,\set{=_s},\Sigma_s}$, strings with the equality predicate;
%%, where $s_1 = s_2$ if and only if $s_1$ and $s_2$ are the same string;
%\item $\typename{real} = \tup{\reals,\set{=_r,<_r},\Sigma_r}$, reals with the usual comparison operators; 
%\item $\typename{int} = \tup{\ints,\set{=_{int},<_{int},succ},\Sigma_{int}}$, integers with the usual comparison operators, as well as the successor predicate.
%\end{inparaenum}


%\todo[inline]{DOUBLE CHECK WHETHER DATA PROPAGATED ON THE OUTGOING ARCS COME ONLY FROM NU OR RELATIONS}
% A \emph{type domain} $\types$ is a finite set of pairwise disjoint \emph{data types} $\type=\tup{\dom_\type,\sigp_\type,\Sigma_\type}$, where a set $\dom_\type$ is a \emph{value domain}, $\sigp_\type$ is a finite set of \emph{predicate  symbols} and $\Sigma_\type$ is the signature interpretation, i.e., a function associating each predicate symbol $S$ of arity $n$, denoted as $S/n$, to an $n$-ary relation $\Sigma(S)\subseteq \dom_\type^n$.
%Examples of data types are:
%\begin{inparaenum}[\it (i)]
%\item $\typename{string} = \tup{\strings,\set{=_s},\Sigma_s}$, strings with the equality predicate;
%%, where $s_1 = s_2$ if and only if $s_1$ and $s_2$ are the same string;
%\item $\typename{real} = \tup{\reals,\set{=_r,<_r},\Sigma_r}$, reals with the usual comparison operators; 
%\item $\typename{int} = \tup{\ints,\set{=_{int},<_{int},succ},\Sigma_{int}}$, integers with the usual comparison operators, as well as the successor predicate.
%\end{inparaenum}
%\todo[inline]{Here, one could compare "our" datatypes with color types in CPN}
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%			CATALOG	       %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
We call $R(a_1:\type_1,\ldots,a_n:\type_n)$ a \emph{$\types$-typed relation schema}, where $R$ is a relation name and $a_i:\type_i$ indicates the $i$-th attribute of $R$ together with its data type. When no ambiguity arises, we omit relation attributes and/or their data types. 
A \emph{$\types$-typed catalog schema} $\schema_\types$ is a finite set of $\types$-typed relation schemas.
A \emph{$\types$-typed catalog $\cat$ over $\schema_\types$} is a finite set of facts of the form $R(\cname{o_1},\ldots,\cname{o_n})$, where 
$R\in \schema$ and $\cname{o_i}\in \dom_{\type_i}$, for $i \in \set{1,\ldots,n}$.
%Given a type $\type \in \types$, the \emph{$\type$-active domain of $\I$}, is the set of $\adom[\type]{\I}=\set{\cname{o} \in \dom_\type\mid \cname{o} \text{ occurs in }\I}$. 

We adopt two types of \emph{constraints} in the catalog relations. First of all, we assume that the first attribute of every relation $R\in\schema_\types$ represents its \emph{primary key}, denoted as $\PK{R}$. Moreover, a type of every primary key attribute should be different from the types of other primary key attributes. Then, for any $R,S\in\schema_\types$, $\FK{R}{a}{S}{id}$ defines that the projection $\proj{R}{a}$ is a \emph{foreign key} referencing $\proj{S}{id}$, where $\PK{S}=id$, $\PK{R}\neq a$ and $\tfun(id)=\tfun(a)$.
While the given setting with constraints may seem a bit too restrictive, it is the one adopted in the most sophisticated settings for data-centric processes where parameterisation of read-only data is tackled \cite{DeLV16,MSCS20}.
 In addition, this matches exactly the representation of read-only relations in \mcmt.

\newcommand{\prodcat}{\relname{ProdCat}}
\newcommand{\producttype}{\datatype{ProdType}}
\newcommand{\compatible}{\relname{Comp}}
\newcommand{\compid}{\datatype{CId}}
\newcommand{\trucktype}{\datatype{TruckType}}


\begin{example}
\label{ex:catalog}
We consider a simple catalog of an order-to-delivery scenario, containing two relation schemas.
The first is a unary relation schema $\prodcat(p:\producttype)$ indicating the product types (such as vegetables, office products, furnitures) available in the catalogue of products of the organisation.
The second is a binary relation schema $\compatible(c:\compid,p:\producttype,t:\trucktype)$  indicating the compatibility between product truck types that can be used to deliver orders; for example, one may specify that vegetables are compatible only with those truck types that comprise a refrigerator. 
\end{example}



\smallskip\noindent
\textbf{Catalog queries.} 
%\todo[inline]{do we support all the data types and related predicates? or shall we go for an abstract domain and inequalities only? like that we'll get conjunctive queries with atomic negation and inequalities!}
Given $\types$, we fix a countably infinite set $\varset$ of typed variables with a \emph{variable typing function} $\vartype: \varset \rightarrow \types$. Such function can be easily extended to account for sets, tuples and multisets of variables as well as constants. 
As the query language we opt for the union of conjunctive queries with inequalities and atomic negations that can be specified in terms of first-order (FO) logic extended with types. This corresponds to the widely investigated fragment of SQL consisting of select-project-join queries with filters, and unions thereof.

A \emph{(well-typed) conjunctive query (CQ) with atomic negation} $Q$ over $\schema_\types$ is a formula of the form: 
\[Q::=\varphi~\mid~R(x_1,\ldots,x_n)~\mid~\neg R(x_1,\ldots,x_n)~\mid~Q_1 \land Q_2~\mid~\exists x.Q,\text{ where}\] 
\begin{inparaenum}[\it(i)]
\item $R(\type_1,\ldots,\type_n)\in\schema$, $x\in\varset$ and each $x_i$ is either a variable of type $\type_i$ or a constant from $\dom_{\type_i}$;
\item $\varphi::=S(y_1,\ldots,y_m)~\mid~\neg\varphi~\mid~\varphi\land\varphi~\mid~\top$ is a \emph{condition} s.t. $S\in\sigp_\type$ and $y_i$ is either a variable of type $\type$ or a constant from $\dom_{\type}$.
\end{inparaenum}
We use $\cqd$ to denote the set of all such conjunctive queries and $\free{Q}$ to denote the set of all free variables (i.e., those not occurring in the scope of quantifiers) of query $Q$. 
%The definition of the $\free$ function can be naturally extended to sets of queries. 
We also use $\conds$ to denote the set of all possible conditions, $\varsin{Q}$ to denote the set of all variables in $Q$ and $\constin{Q}$ the set of all constants in $Q$.
%A \emph{boolean query} is a query without free variables. 
With $\ucqd$ we denote the set off all \emph{unions of conjunctive queries} over $\schema_\types$, where each query $Q\in\ucqd$ is defined as $Q=\bigwedge_{i=1}^n Q_i$, with $Q_i\in\cqd$. 
%%%% Commented by Marco
%Finally, given a query $Q$ with name $\mathtt{q}$ and such that $\free{Q} = \set{x_1, \ldots , x_n}$, we employ notation $\query{q}{x_1,\ldots,x_n}{Q}$ to explicitly indicate the free variables of $Q$, and to fix a natural ordering over them.
 
A \emph{substitution} for a set $X = \set{x_1,\ldots,x_n}$ of typed variables
is a function $\subst: X \rightarrow \dom_\types$, such that
$\subst(x) \in \dom_{\vartype(x)}$ for every $x \in X$. An empty substitution is denoted as $\tup{}$.  A \emph{substitution $\subst$ for a query $Q$}, denoted as $Q\subst$, is a substitution for variables in $\free{Q}$. 
%We denote by $Q\subst$ the boolean query obtained from $Q$ by replacing
%each occurrence of a free variable $x \in \free{Q}$ with the value $\subst(x)$.
%
An \emph{answer to a query $Q$} in a catalog $\cat$ is a set of substitutions $\ans(Q,\cat) = \{ \subst: \free{Q} \rightarrow \val(\cat) \mid
\qent{\cat}{\subst}{Q}\}$, where $\val(\cat)$ denotes the set of all constants occurring in $\cat$ and $\models$ denotes standard FO entailment. 
%Given a $\types$-typed database schema $\schema$, a $\types$-typed instance
%$\I$ over $\schema$, and a \fod query $Q$ over $\schema$, the set of
%\emph{answers} to $Q$ in $\I$ is defined as the set
%$\ans(Q,\I) = \{ \subst: \free{Q} \rightarrow \adom[\types]{\I} \mid
%\qent{\I}{\subst}{Q}\}$ of substitutions for $Q$, where $\models$ denotes
%standard FO entailment (i.e., we use \emph{active-domain semantics}).
%%%
%
%When $Q$ is boolean, we shall write $\ans(Q,\I) \equiv \true$ if $\ans(Q,\I)=\set{\tup{}}$ , and $\ans(Q,\I) \equiv \false$ if $\ans(Q,\I) = \emptyset$.
%Boolean queries are also used to express \emph{constraints} over $\schema$.  

\begin{example}
\label{ex:queries}
Consider the catalog of Example~\ref{ex:catalog}. Query $\prodcat(p)$ retrieves the product types $p$ present in the catalog, whereas given a product type value $\cval{v}$, query $\exists c.\compatible(c,\cval{v},t)$ returns the truck types $t$ compatible with $\cval{v}$.
\end{example}



%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%			MULTISETS       %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%			SYNTAX	       %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\medskip
\noindent
\textbf{\clognets.} Before defining the central notion of \clognet, we fix some standard notions related to \emph{multisets}. Given a set $A$,  the \emph{set of multisets} over $A$, written $\mult{A}$, is the set of mappings of the form $m:A\rightarrow \mathbb{N}$.
Given a multiset $S \in \mult{A}$ and an element $a \in A$, $S(a) \in \mathbb{N}$ denotes the number of times $a$ appears in $S$.  Given $a \in A$ and $n \in \mathbb{N}$, we write $a^n \in S$ if $S(a) = n$.  The support of $S$ is the set of elements that appear in $S$ at least once: $\supp{S} = \set{a\in A\mid S(a) > 0}$. We also consider the usual operations on multisets. Given $S_1,S_2 \in \mult{A}$:
\begin{inparaenum}[\it (i)]
\item $S_1 \subseteq S_2$ (resp., $S_1 \subset S_2$) if $S_1(a) \leq S_2(a)$ (resp., $S_1(a) < S_2(a)$) for each $a \in A$;
\item $S_1 + S_2 = \set{a^n \mid a \in A \text{ and } n = S_1(a) + S_2(a)}$;
\item if $S_1 \subseteq S_2$, $S_2 - S_1 = \set{a^n \mid a \in A \text{ and } n = S_2(a) - S_1(a)}$;
\item given a number $k \in \mathbb{N}$, $k \cdot S_1 = \set{a^{kn} \mid a^n \in S_1}$;
\item $|m|=\sum_{a\in A}m(a)$.
\end{inparaenum}
A multiset over $A$ is called empty (denoted as $\mult\emptyset$) iff $\mult\emptyset(a)=0$ for every $a\in A$.


We are now ready to define \clognets, extending the formalism of \nucpns with the ability of querying a read-only catalog. In the spirit of CPNs, a \clognet net assigns to each place a color type, which in turn corresponds to a data type or to the cartesian product of multiple data types from $\types$. 
Contents of places can be referenced via \emph{inscriptions} -- tuples of variables and constants. We denote by $\Omega_A$ the set of all possible inscriptions over a set $A$ and, with slight abuse of notation, use $\varsin{\omega}$ (resp., $\constin{\omega}$) to denote the set of variables (resp., constants) of $\omega\in\Omega_A$.
To account for fresh external inputs, we employ the well-known mechanism adopted in $\nu$-Petri nets~\cite{RVFE11} and introduce a countably infinite set $\nuvarset$ of $\types$-typed \emph{fresh variables}, where for every $\nu \in \nuvarset$, we have that $\dom_{\vartype(\nu)}$ is countably infinite (this provides an unlimited supply of fresh values). Hereafter, we fix a countably infinite set of $\types$-typed variable $\vars = \varset \uplus \nuvarset$ as the disjoint union of ``normal" variables $\varset$ and fresh variables $\nuvarset$. 

\begin{definition}
\label{def:clognet}
A $\types$-typed \clognet $\net$ over a catalog schema $\schema_\types$ is a tuple  
$(\types, \schema_\types, \places,\transitions,\inflow,\outflow,\coloring,\guass)$, where:
\begin{compactenum}
%
%\item $(\places,\transitions,\flow)$ is a net structure;
\item $\places$ and $\transitions$ are finite sets of places and transitions, s.t. $P\cap T=\emptyset$;
%
\item $\coloring: \places \rightarrow \powerset(\types)$ is a place typing function;
%\item $\quass: \vplaces \rightarrow \ucqd$ is a query assignment function, s.t. $\vartype(\free{\quass(p)})=\coloring(p)$ for every $p\in\vplaces$;
%mapping each view place $p \in \vplaces$ with $\coloring(p) = \type_1\times\ldots\times\type_n$ to a query $Q(x_1,\ldots,x_n)$ from $\queries$, s.t. the color of $p$ component-wise matches with the types of the free variables in $Q$: for each $i \in \set{1,\ldots,n}$, we have $\type_i = \vartype(x_i)$.
%
\item $\inflow: \places \times \transitions \rightarrow \mult{\Omega_{\varset}}$ is an input flow, 
%assigning multisets of inscriptions to input arcs, 
s.t. $\vartype(\inflow(p,t))=\coloring(p)$ for every $(p,t)\in\places\times\transitions$;
\item $\outflow: \transitions \times \places \rightarrow \mult{\tuples{\vars \cup \dom_\types}}$ is an output flow, s.t. $\vartype(\outflow(t,p))=\coloring(p)$ for every $(t,p)\in\transitions\times\places$;
%each of such inscriptions $\omega$ is compatible with each of its input places $p$, i.e., for every $i \in \set{1,\ldots,m}$, we have $\vartype(x_i) = \type_i$, where $\coloring(p) = \type_1 \times \ldots\times \type_m$.
%

\item $\guass:  \transitions \rightarrow \set{Q\land \varphi\mid Q\in\ucqd, \varphi\in\conds}$ is a partial guard assignment function, s.t., for every $\guass(t)=Q\land\varphi$ and $t\in\transitions$, the following holds:  
\begin{compactenum}
	\item $\varsin{\varphi}\subseteq\invars{t}$, where $\invars{t}=\cup_{p\in\places}\varsin{\inflow(p,t)}$;
	\item $(\varsin{Q}\cap \outvars{t})\setminus\invars{t}\neq\emptyset$ and $\varsin{Q}\subseteq \varsin{t}$, where $\outvars{t}=\cup_{p\in\places}\varsin{\outflow(t,p)}$ and $\varsin{t}=\invars{t}\cup\outvars{t}$.
	%we do the conditions in this way so as to show that some values in the outgoing arc inscritpions are getting propagated using query answers; however, they're not subsumed as there can be also fresh variables not provided by Q;
	%we should also make sure that free variables of Q are exhaustively covered by the variables in the input and output arcs  (this is needed for the translation, but also makes sense from the modelling point of view: why to write queries whose results you're not going to use?)
\end{compactenum}

%
\end{compactenum}
%
\end{definition}
%\todo[inline]{Define a unique flow relation and arc labeling for inscriptions (more old-schoolish)}

Here, the role of guards is twofold. On the one hand, similarly, for example, to CPNs, guards are used to impose \emph{conditions} (using $\varphi$) on tokens flowing through the net. On the other hand, a guard of a transition $t$ may also \emph{query} (using $Q$) the catalog in order to propagate some data into the net. The acquired data may be still filtered by using $\invars{t}$. Note that in condition \emph{(b)} of the guard definition we specify that there are some variables (excluding the fresh ones) in the outgoing arc inscriptions that do not appear in $\invars{t}$ and that are used by $Q$ to insert data from the catalog. Moreover, it is required that all free variables of $Q$ must coincide with the variables of inscriptions on outgoing and incoming arcs of a transition it is assigned to.
In what follows, we shall define arc inscriptions as $k\cdot\omega$, where $k\in\naturals$ and $\omega\in\Omega_A$ (for some set $A$). 



\smallskip
\noindent
\textbf{Semantics.}
The execution semantics of a \clognet is similar to the one of CPNs. Thus, as a first step we introduce the standard notion of net marking. 
Formally, a \emph{marking} of a \clognet $N=(\types, \schema_\types, \places,\transitions,\inflow,\outflow,\coloring,\guass)$ is a function $m:\places\rightarrow \mult{\Omega_\types}$, so that  $m(p)\in\mult{\dom_{\coloring(p)}}$ for every $p\in\places$. 
%and  $m(v)=\ans(\quass(v),\cat)$ for every $v\in\vplaces$. The latter requirement guarantees that $m$ is \emph{aligned} to $\cat$ via $\quass$. 
We write $\marked{N}{m}$ to denote \clognet $N$ marked with $m$. We use symbol $m_0$ to define the initial marking of the net.

The firing of a transition $t$ in a marking is defined w.r.t.~a so-called \emph{binding} for $t$ defined as $\sigma : \varsin{t} \rightarrow \types$. Note that, when applied to (multisets of) tuples, $\sigma$ is applied to every variable singularly. 
For example, given $\sigma=\set{x\mapsto 1, y\mapsto \cname{a}}$, its application to a multiset of tuples $\omega=\set{\tup{x,y}^2,\tup{x,\cname{b}}}$ results in $\sigma(\omega)=\set{\tup{1,\cname{a}}^2,\tup{x,\cname{b}}}$.
%\todo[inline]{Do more precise $\sigma$ notation}
\begin{definition}
\label{def:trans_e}
A transition $t \in\transitions$ is \emph{enabled} in a marking $m$, written $\enabled{m}{t}$, iff there exists a binding $\sigma$ and the following conditions hold:
\begin{inparaenum}[\it (1)]
\item  $ \sigma(\inflow(p,t))\subseteq m(p)$, for every $p\in\places$;
\item $\sigma(\guass(t))$ is true;
\item $\sigma(x)\not\in \val(m)\cup \val(\cat)$, for
every $x\in\nuvarset \cap \outvars{t}$.\footnote{Here, with slight abuse of notation, we define by $\val(m)$ the set of all values appearing in $m$. }
% ($\sigma$ assigns globally fresh values to fresh variables in the expressions attached to arcs outgoing from $t$).
\end{inparaenum}
\end{definition}
When a transition $t$ is enabled, it may fire. Next we define what are the effects of firing a transition with some binding $\sigma$.
%Its firing with some binding has then a twofold effect. First, all tokens present in input places of $t$ that match inscriptions on corresponding arcs are consumed. Second, tokens built after the inscriptions on output arcs are produced and put into target places.

\begin{definition}
\label{def:trans_f}
Let $\marked{N}{m}$ be a marked \clognet and $t\in\transitions$ is a transition enabled in $m$ with some binding $\sigma$. Then, $t$ may \emph{fire} producing a new marking $m'$, such that $m'(p)=m(p)-\sigma(\inflow(p,t))+\sigma(\outflow(t,p))$ for every $p\in\cplaces$. We denote this as $\fire{m}{t}{m'}$ and assume that the definition is inductively extended to sequences $\tau\in\transitions^*$.
\end{definition}
For $\marked{N}{m_0}$ we use $\mathcal{M}(N)=\set{m\mid \exists \tau\in\transitions. \fire{m_0}{\tau}{m}}$ to denote the set of all markings of $N$ reachable from its initial marking $m_0$. 

With these notions in place, the execution semantics of a marked \clognet $\marked{N}{m}$ is defined in terms of a possibly infinite-state transition system in which states are labeled by reachable markings and each arc (or transition) corresponds to the firing of a transition in $N$ with a given binding. The transition system captures all possible executions supported by the net, by interpreting concurrency as interleaving.

Technically, the execution semantics of the marked \clognet $\marked{N}{m_0}$ is captured by transition
system $\tsys{N}=(S, s_0, \trans)$, where:
\begin{compactitem}[$\bullet$]
\item $S$ is a possibly infinite set of makrings over $N$;
\item $\trans\subseteq S\times \transitions \times S$ is a $\transitions$-labelled transition relation between pairs of markings;
\item $S$ and $\trans$ are defined by simultaneous induction as the smallest sets satisfying the following conditions:
\begin{inparaenum}[\it(i)]
\item $m_0\in S$;
\item given $m\in S$, for every transition $t\in\transitions$, binding $\sigma$ and marking $m'$ over $N$, if $\fire{m}{t}{m'}$, then $m'\in S$ and $m\overset{t}{\trans} m'$.
\end{inparaenum}
\end{compactitem}

We close with an example that illustrates all the main features of \clognets.



\begin{example}
\label{ex:clognet}
Starting from the catalog in Example~\ref{ex:catalog}, Figure~\ref{fig:clognet} shows a simple, yet sophisticated example of \clognet capturing the following order-to-delivery process. Orders can be created by executing the \transition{new order} transition, which uses a $\nu$-variable to generate a fresh order identifier. A so-created, working order can by populated with items, whose type is selected from those available in the catalog relation $\prodcat$. Each item then carries its product type and owning order. When an order contains at least one item, it can be paid. Items added to an order can be removed or loaded in a compatible truck. The set of available trucks, indicating their plate numbers and types, is contained in a dedicated \emph{pool} place. Trucks can be borrowed from the pool and placed in house. An item can be loaded into a truck if its owning order has been paid, the trucks is in house, and the truck type and product type of the item are compatible according to the $\compatible$ relation in the catalog. Items from the same and different orders can be loaded in a truck, and while the truck is in house, they can be dropped from the truck, which makes them ready to be loaded again. A truck can be driven for delivery if it contains at least one loaded item. Once the truck is at destination, some items may be delivered (this is simply modelled non-deterministically, without explicitly inspecting whether the reached destination matches with the delivery address reached by the truck).  The truck can then either move, or go back to the company headquarters. 
\end{example}

\begin{figure}[t!]

\tikzstyle{truck}=[draw=violet]
\tikzstyle{order}=[draw=cyan]
\tikzstyle{item}=[draw=orange]
\tikzstyle{mytrans}=[transition,font=\scriptsize,minimum width=10mm]

\newcommand{\order}{\datatype{Order}}
\newcommand{\barcode}{\datatype{BarCode}}
\newcommand{\oitem}{\datatype{Item}}
\newcommand{\plate}{\datatype{Plate}}
\newcommand{\truck}{\datatype{Truck}}

\centering
\resizebox{\textwidth}{!}{
\begin{tikzpicture}[->,>=stealth',auto,x=15mm,y=1.0cm,node distance=20mm and 15mm,thick]



\node[place,truck] (pool) {};
\node[below=-1mm of pool] {
  \begin{tabular}{@{}c@{}}
    pool\\
    $\truck$  
  \end{tabular}
};

\node[mytrans,right=10mm of pool,truck] (use) {\transition{use}};

\node[place,right=of use,truck] (inhouse) {};
\node[below=-1mm of inhouse] {
  \begin{tabular}{@{}c@{}}
    in house\\
    \truck  
  \end{tabular}
};


\node[mytrans,right=of inhouse,truck] (goback) {\begin{tabular}{@{}c@{}}\transition{go}\\\transition{back}\end{tabular}};


\node[mytrans,above=5mm of goback,truck] (drive) {\transition{drive}};

\node[place,right=of goback,truck] (atdest) {};
\node[below=-1mm of atdest] {
  \begin{tabular}{@{}c@{}}
    at dest\\
    \truck  
  \end{tabular}
};

\node[mytrans,right=10mm of atdest,truck] (move) {\transition{move}};




  \node[mytrans,above=20mm of pool,item] (ai) {
    \begin{tabular}{@{}c@{}}
      \transition{add}\\      
      \transition{item}
    \end{tabular}
  };
  \node[left=0mm of ai] {\footnotesize $\left[\prodcat(p)\right]$};
  
  \node[mytrans,below=5mm of ai,item] (remove) {\transition{rem}};
    
  \node[place,right=10mm of ai,item] (ready) {};
  \node[below=-1mm of ready] {
    \begin{tabular}{@{}c@{}}
      ready\\
      \oitem  
    \end{tabular}
  };
  
  \node[mytrans,right=of ready,item] (load) {\transition{load}};
  \node[above=0mm of load] (loadguard) {\footnotesize$[\exists c.\compatible(c,p,t)]$};
  
  \node[mytrans,below=5mm of load,item] (drop) {\transition{drop}};
  
  
  \node[place,right=of load,item] (intruck) {};
  \node[above=-1mm of intruck] {
    \begin{tabular}{@{}c@{}}
      in truck\\
      $\oitem\times\plate$  
    \end{tabular}
  };
  
  
  \node[mytrans,right=of intruck,item] (deliver) {\transition{deliver}};

  \node[place,right=10mm of deliver,item] (delivered) {};
  \node[below=-1mm of delivered] {
    \begin{tabular}{@{}c@{}}
      delivered\\
      \oitem  
    \end{tabular}
  };



  \node[place,above=10mm of ai,order] (inprep) {};
  \node[above=-1mm of inprep] {
    \begin{tabular}{@{}c@{}}
      working\\
      \order  
    \end{tabular}
  };

  \node[mytrans,left=10mm of inprep,order] (new) {
    \begin{tabular}{@{}c@{}}
    \transition{new}\\
    \transition{order}  
    \end{tabular}
  };


  \node[mytrans,above=10mm of ready,order] (pay) {\transition{pay}};  
  \node[place,right=of pay,order] (paid) {};
  \node[above=-1mm of paid] {
    \begin{tabular}{@{}c@{}}
      paid\\
      \order  
    \end{tabular}
  };



\draw[truck,->] (pool) --node[below]{$\tup{m,t}$} (use);
\draw[truck,->] (use) --node[below]{$\tup{m,t}$} (inhouse);
\draw[truck,->] (inhouse) --node[below,xshift=4mm,yshift=2mm]{$\tup{m,t}$} (drive);
\draw[truck,->] (drive) --node[below,xshift=-4mm,yshift=2mm]{$\tup{m,t}$} (atdest);
\draw[truck,->] (atdest) --node[below]{$\tup{m,t}$} (goback);
\draw[truck,->] (goback) --node[below]{$\tup{m,t}$} (inhouse);
\draw[truck,<->] (atdest) --node[below]{$\tup{m,t}$} (move);
  
  
\draw[->,item,sloped] (ready) --node[yshift=-1mm,above]{$\tup{p,o}$} (remove);
\draw[->,item] (ready) --node{$\tup{p,o}$} (load);
\draw[<->,truck,out=135,in=-135] (inhouse) edge node{$\tup{m,t}$} (load);

\draw[->,item,sloped] (intruck) --node[above,yshift=-1mm]{$\tup{p,o,m}$} (drop);
\draw[->,item,sloped] (drop) --node[above,yshift=-1mm,xshift=-2mm]{$\tup{p,o}$} (ready);
\draw[<->,truck] (inhouse) --node[right]{$\tup{m,t}$} (drop);

\draw[->,item] (load) --node{$\tup{p,o,m}$} (intruck);
\draw[->,item] (intruck) --node{$\tup{p,o,m}$} (deliver);
\draw[<->,item] (drive) edge node[right]{$\tup{p,o,m}$} (intruck);

\draw[<->,truck] (atdest) --node{$\tup{m,t}$} (deliver);
\draw[->,item] (deliver) --node{$\tup{p,o}$} (delivered);

\draw[->,order] (new) --node{$\nu_o$} (inprep);
\draw[->,order] (inprep) --node{$o$} (pay);
\draw[->,order] (pay) --node{$o$} (paid);

\draw[<->,order] (inprep) --node{$o$} (ai);
\draw[->,item] (ai) --node{$\tup{p,o}$} (ready);
\draw[<->,item] (ready) --node{$\tup{p,o}$} (pay);
\draw[<->,order] (loadguard) edge node{$o$} (paid);
  
\end{tikzpicture}
}
\caption{An order-to-delivery \clognet. The net catalog is shown in Example~\ref{ex:catalog}. In the picture, $\oitem$ and $\truck$ are compact representations for $\producttype \times \order$ and $\plate \times \trucktype$ respectively. The top blue part refers to orders, the central orange part to items, and the bottom violet part to delivery trucks.}
\label{fig:clognet}
\end{figure}

Example~\ref{ex:clognet} shows various key aspects related to modelling data-aware processes with multiple case objects using \clognets. First of all, whenever an object is involved in a many-to-one relation from the ``many'' side, it then becomes responsible of carrying the object to which it is related. This can be clearly seen in the example, where each item carries a reference to its owning order and, once loaded into a truck, a reference to the truck plate number. 

Secondly, the three object types involved in the example show three different modelling patterns for their creation. Unboundedly many orders can be genuinely created using a $\nu$-variable to generate their (fresh) identifiers. The (finite) set of trucks available in the domain is instead fixed in the initial marking, by populating the \emph{pool} place. The \clognet clearly shows that such trucks are used as resources which can change state but are never destroyed nor created. Finally, the case of items is particularly interesting. Items in fact can be arbitrarily created and destroyed. However, their creation is not modelled using an explicit $\nu$-variable, but is instead simply obtained by the \transition{add item} transition with the usual token-creation mechanism of standard (non-coloured) Petri nets. Thanks to the multiset semantics of Petri nets, it is still possible to create multiple items having the same product type and owning order. However, it is not possible to track the evolution of a specific item, since there is no explicit identifier carried by item tokens. This is not a limitation in this example, since items are not referenced by other objects present in the net (which is instead the case for orders and trucks). All in all, this shows that $\nu$-variables are only necessary when the \clognet needs to handle the arbitrary creation of objects that have to be referenced by other objects, which in this net is only the case for orders.



%\todo[inline]{Bounded???}
%
%\begin{definition}
%Given $b\in\naturals$, a marked \clognet $\marked{N}{m_0}$ is called \emph{bounded with bound $b$} if $|m(p)|\leq b$, for every marking $m\in\mathcal{M}(N)$ and every place $p\in\cplaces$. 
%\end{definition}
%%In this work we are going to consider \clognets which assume a bound on their control places only. 
%Note that, even though a number of tokens in every place of a bounded \clognet is finite, a transition system representing all its possible executions is  going to have potentially infinitely many states.  




==> 3-array-based-systems.tex <==
\section{Array-based systems}
\todo[inline]{is it even needed? does it make sense to introduce abstractly what array-based systems are?}

==> 4-translation_bounded.tex <==
\section{From \clognets to MCMT}



\todo[inline]{as many approaches try to study data as business artifacts, we follow the same line and say that, in general, the data we use come from a relatively abstract object domain where we can explicitly talk about components of objects (a-la relations), provide them with unique identities (a-la primary keys) and explicitly specify dependencies between them (a-la foreign-keys)}
\todo[inline]{our formalism is directly subsumed by the class of db-nets studied before. however, verification of db-nets is a hard task and, so far, none has studied any kind of more practical verification tasks for that formalism considering only its state-boundedness restriction. as a matter of fact, there is a conjecture saying that it is possible to acquire decidability of a FO variant of $\mu$-calculus for db-nets using a reduction to another foramlism of data-centric dynamic systems, by analogy with the work done on $\nu$-Petri nets. again, in this work we depart from an existing verification technique that we consider expressive and robust enough to conduct different analytic tasks intrinsic to the BPM domain. to this end, we isolate a subclass of db-nets, called \clognets and demonstrate how it can be encoded into a formalism used behind the MCMT technique. moreover, we give an example of how one can formalize business policies such as data-aware soundness on top of such nets as properties and how such properties are getting directly translated into the MCMT language.}
\todo[inline]{for this work we're going to use a setting of \mcmt working for data-aware processes called MCMT for Data-driven Applications}
Now we show how to translate a bounded \clognet $\marked{N}{m_0}$ with a fixed bound $b\in\naturals$, where $N=(\types, \schema_\types, \places,\transitions,\inflow,\outflow,\coloring,\quass,\guass)$,  into a corresponding \mcmt specification. The translation process is going to be split into two phases. First, we walk one through the representation of the type domain and catalog in \mcmt. Note that all the data components of our formalism as well as the query language were intended to have a design allowing for their seamless representation in \mcmt.
Second, we demonstrate a step-wise process of encoding of the \clognet transition enablement using array-based systems. To this end, we show on a single transition how to generate bindings based on the net marking and the content of the catalog provided by the view place queries. Finally, we encode the transition firing and new marking generation based on the acquired bindings. 




\textbf{Data and schema translation.} We start by describing how to translate static data-related components. 
\begin{compactenum}
%first - data types
\item Let  $\types=\set{\type_1,\ldots,\type_{n_d}}$. Then, every data type $\type_i$ has to be represented as a corresponding sort in \mcmt using the following declaration
\begin{mc}
	:smt (define_type Di)
\end{mc}
For every declared data type $\type$, \mcmt automatically generates a special NULL constant is used to define an empty (or undefined) value of $\type$.
We recall that \mcmt does not only support user-defined data types, but also user-defined operations. However, in this paper we only consider the former and assume that every type has an equality operation defined for it. For more details on user defined operations please refer to the \mcmt documentation. \todo{cite the documentation and, if needed, remove this paragraph}
%second - relations
\item To represent the catalog relations of $\schema_\types=\set{R_1,\ldots,R_{n_r}}$ in \mcmt, we need to follow the next steps. Recall that in catalog every relation schema has $n+1$ typed attributes among which some may be foreign keys referencing other relations, its first attribute is a primary key, and, finally, primary keys of different relation schemas have different types. Having these conditions in mind, we adopt a functional characterization of read-only databases studied in \cite{CGGMR19} for specifying relations in the catalog. 
For every relation $R_i(id,A_1,\ldots,A_n)$, where $\PK{R}=\set{id}$, we introduce unary functions that correctly reference each attribute of $R_i$ using its primary key. More specifically, for every $A_j$ ($j=1,\ldots,n$) we create a function $f_{R_i,A_j}:\dom_{\vartype(id)}\rightarrow\dom_{\vartype{A_j}}$. If $A_j$ is referencing an identifier of some other relation $S$ (i.e., $\FK{R_i}{A_j}{S}{id}$), then $f_{R_i,A_j}$ represents the foreign key referencing to $S$. Note that in this types of $A_j$ and $id$ should coincide. In \mcmt, assuming that $\texttt{id\_D}=\vartype(id)$ and $\texttt{Aj\_D}=\vartype(A_j)$, this is going to look as follows:
\begin{mc}
	:smt (define Ri_Aj ::(-> id_D Aj_D))
\end{mc}
%third - constants 
\item All the constant appearing in all the net-related components must be recorded. Let $C=\set{v_1,\ldots,v_{n_c}}$ be a set of all constants appearing in $N$. $C$ is defined as $\bigcup_{t\in\transitions}\constin{\guass(t)}\cup\supp{m_0}\cup\bigcup_{t\in\transitions,p\in\cplaces} \constin{\outflow(t,p)}$. Then, every constant $v_i\in C$ of type $\type$ has to be explicitly declared in \mcmt:
\begin{mc}
	:smt (define vi ::D)
\end{mc}
\end{compactenum}







%We also introduce a condition that would allow us to check whether a tuple $(x_0,\ldots,x_n)$ belongs to a relation $R$ with key dependencies on attributes $A_1$,\ldots,$A_n$:
%\[R(x_0,\ldots,x_n) \text{\,iff\,} x_0 \neq\nullv \land x_1 =f_{R,A_1}(x_0)\land \ldots\land x_n =f_{R,A_n}(x_0)\]

%\todo[inline]{do we treat sorts abstractly or shall we use more concrete sorts? (e.g., cartesian product)} 

At the end, all the aforementioned declared elements have to be repeated in a special declaration used by \mcmt in the database-driven mode:
\begin{mc}
	:db_driven
	:db_sorts D1, ..., Dnd
	:db_functions R1_A1, ..., Rnr_Ak
	:db_constants v1, ..., vnc
\end{mc}

\textbf{Places.} Given that every control place  along the net run is going to store at most $b$ tokens, we do not need to ensure a potentially infinite provision of values to $p$ using unbounded arrays and thus can simply use boundedly many variables. More specifically, for every place $p\in\cplaces$ with $\coloring(p)=\type_1\times\ldots\times\type_k$, we are going to introduce a $b\times k$ ``matrix'' of variables such that every row potentially stores values for each of $k$ components of some token in $p$.  In \mcmt, such variables are declared as global arrays:
\begin{mc}
	:global p_11 D1
	...
	:global p_1k Dk
	:global p_21 D1
	...
	:global p_bk Dk
\end{mc} 
Then, intuitively, a $j$-th token $(v_1,\ldots,v_k)\in m(p)$, where $0\leq j \leq b$, can be seen a conjunction of equalities $p_{j_1}=v_1,\land\ldots\land\,p_{j_k}=v_k$. Using this intuition and assuming that , we are going to represent the initial marking $m_0$ with the following special \mcmt initialization statement:

\begin{mc}
	:initial
	:var
	:cnj $mp_1$ ... $mp_n$
\end{mc}
Here, \texttt{cnj} represents a conjunction of atomic equations that, for ease of reading, we organized in blocks, where each $mp_i$ encodes $m_0(p_i)$, for $p_i\in\cplaces$ with $\coloring(p_i)=\type_1\times\ldots\times \type_k$. Given that the amount of tokens in every places is bounded, we shall initialize every raw in the matrix of variables of every place by using either values of the tokens or special NULL constants. 
Now, if $m_0(p_i)\neq\mult\emptyset$, then a $j$-th token $(v_1,\ldots,v_k)\in m_0(p_i)$ is going to be represented in $mp_i$ using the following conjunction:  
\begin{mc}
	(= pi_j1 v_1)(= pi_j2 v_2)...(= pi_jk v_k) 
\end{mc}
If $p_i$ has no tokens or $|m_0(p_i)|<b$, then all the related place variables are instantiated using NULL constants of the respective type. More specifically, the initialization statement for missing tokens is composed of the following conjunction:
\begin{mc}
(= pi_j1 NULL_D1)(= pi_j2 NULL_D2)...(= pi_jk NULL_Dk) 
\end{mc}

View places are not translated into the corresponding place objects. Given that their content remains unchanged during the net execution, there is no need to represent them explicitly. Instead, view places should be seen as a part of transition guards that have access to an external data storage via queries which, in what follows, are going to be incorporated into \mcmt transition guards.


\begin{figure}[t!]
\centering
\resizebox{.72\hsize}{!}{
\begin{tikzpicture}[->,>=stealth',auto,x=1.3cm,y=1.0cm,thick]

   \node[transition,label={below:\large $t$}] (t) at (3,0) {~~~~\phantom{x}~~~~};
   	\node[above of = t, yshift=-.8cm,label=\large $\mathbf{[}{\color{mgreen}G(\vec{y})}\mathbf{]}$]  (guard)  {};

    \viewplace{vp1}{(1.8,-1.4)}{below:\large $V_1$};
    \node[label=\tiny{$\bullet \bullet \bullet$}]  (dots1) at (3,-1.7) {};
    \viewplace{vpm}{(4.2,-1.4)}{below:\large $V_m$};
	
	\node[left=0mm of vp1]  (vq1) 
	  {\large $\cname{Q}_{\cname{V_1}} (\vec{x}_1)$};
    \node[right=0mm of vpm]  (vqm)
      {\large $\cname{Q}_{\cname{V_m}} (\vec{x}_m)$};
	
	\node[place,left of=t,xshift=-3cm,yshift=1.3cm,label={left:\large $pin_1$}] (pin_1) {};
	\node[place,left of=t,xshift=-3cm,yshift=-0cm,label={left:\large $pin_k$}] (pin_k) {};
	\node[left of=t,xshift=-3cm,yshift=.3cm,label=\tiny{$\bullet \bullet \bullet$}]  (dots2) {};

	\node[place,right of=t,xshift=3cm,yshift=1.3cm,label={right:\large $pout_1$}] (pout_1) {};
	\node[place,right of=t,xshift=3cm,yshift=-0cm,label={right:\large $pout_n$}] (pout_n) {};
	\node[right of=t,xshift=3cm,yshift=.3cm,label=\tiny{$\bullet \bullet \bullet$}]  (dots3) {};

	
	
  \path[]
    (pin_1) edge node[above,xshift=-1mm,sloped] {\large $\cname{ri_1}\cdot\vec{in_1}$} (t)    
    (pin_k) edge node[below,xshift=-1mm,sloped] {\large $\cname{ri_k}\cdot\vec{in_k}$} (t)
    (t) edge node[above,xshift=-1mm,sloped] {\large $\cname{ro_1}\cdot\vec{out_1}$} (pout_1)    
    (t) edge node[below,xshift=-1mm,sloped] {\large $\cname{ro_n}\cdot\vec{out_n}$} (pout_n)
    ;
 
    \path[-]
	(vp1) edge node[right,xshift=-1.5mm,yshift=-2.4mm] {\large $\vec{x}_1$} (t) %($(t.north)-(.3,0)$)
	(vpm) edge node[left,xshift=1.5mm,yshift=-2.4mm] {\large $\vec{x}_m$} (t)
	;
\end{tikzpicture}}
\caption{A generic \clognet transition accessing multiple view places, where every $\cname{i_j}$ (resp. $\cname{o_j}$) is a natural number}
\label{fig:t-generic}
\end{figure}


\textbf{Checking transition enablement and generating a new marking.} Now let us show how to represent the transition enablement check as well as effect computation of a fired transition in \mcmt. Assume a transition $t\in\transitions$ depicted in Figure~\ref{fig:t-generic}. The firing of this transition is subject to the following conditions: 
\begin{inparaenum}[\it (1)]
\item there is a binding $\sigma$ that correctly matches tokens in the places to the corresponding inscriptions on the input arcs, and computes new and possibly fresh values that are pairwise distinct from each other as well as from all other values in the marking;
\item each place $pin_i$ provides enough tokens required by a corresponding inscription $F(pin_i,t)=\vec{in_i}$;
\item the guard is satisfied under the selected binding;
\item all the newly computed values are correctly assigned to corresponding variables in $\outvars{t}\setminus\invars{t}$.
\end{inparaenum} 

Condition \textit{(1)} also considers a case when a token component must match the same token component coming from a view place. This has to be taken into consideration as view places are not represented explicitly (i.e., we cannot directly resort to their marking), but their queries are. Thus, for every relation in query $\cname{Q}_{\cname{V_i}}$ 



\textbf{Constructing bindings.}
We have to take into account a case of arc inscriptions causing implicit ``joins'' between the net marking and data retrieved from the catalog. This happens when for two inscriptions $\cname{ri_j}\cdot\vec{in_j}=\inflow(pin_j,t)$ and $\vec{x_i}=\inflow(V_i,t)$ there are some variables $\mathbf{s}:=\set{s_1,\ldots, s_r}$ shared by both of these inscriptions. For ease of presentation, we introduce a function $\pi$ that can define a position of a given variable in a tuple or a relation. For example, $\pi(\tup{x,y,z},y)=2$ or $\pi(R,B)=3$, where $R(id,A,B,E)$.
Then, for every relation $R$ in $\cname{Q_{V_i}}(\vec{x_i})$ generate a formula $\phi_R:=\bigwedge_{s\in\bigl(\mathbf{s}\cap\varsin{R}\bigr)}pin_{j,i_{\pi(\vec{in_j},s)}}=R[\pi(R,s)]$. This formula guarantees that values provided by a constructed binding respect the aforementioned case.

\textbf{Queries}.
For ease of presentation, we assume that every $\cname{Q_{V_i}}$ is represented as a conjunction of atoms (or their negations). Indeed, $\cname{Q_{V_i}}$ can be converted into an equivalent query $\cname{Q'_{V_i}}$ in disjunctive normal form (resulting in existentially quantified disjuncts).
We call an \emph{extended query} a query $Q$ in which every relation has been substituted with its array-based counterpart. More specifically, every relation $R(x_1,\ldots,x_n)$ from $Q$ is going to be substituted with a conjunction 






                         
\endinput
In case of unbounded nets, we need to represent places using arrays. To this end, every place every place $p\in\cplaces$ with $\coloring(p)=\type_1\times\ldots\times\type_k$ is going to be represented as a combination of arrays $p_1,\ldots,p_k$, where a special index type $\typename{P_{ind}}$ with domain $\dom_{P_{ind}}$ is used as the array index sort and $\type_1,\ldots,\type_k$ account for the respective target sorts of the aforementioned arrays. In \mcmt this is provided by the following declaration:
\begin{mc}
:local $p_1$ $D_1$
$\ldots$
:local $p_k$ $D_k$
\end{mc} 
Then, intuitively, given $(v_1,\ldots,v_k)\in m(p)$, we associate to it an element $e\in\dom_{P_{ind}}$ and a tuple $(e,p_1[e],\ldots,p_k[e])$, where $p_1[e]=v_1,\ldots, p_k[e]=v_k$. Here, $e$ is an internal identifier of this tuple  in $m(p)$.

to get a $e$'th token in a place $p$, one needs to write 
\textbf{What about the index sort? It has to coincide with the one from the read-only DB --> thus all the place colors should contain IDs!}

==> 4-translation_old.tex <==
\section{From \clognets to MCMT}

\todo[inline]{recent research reveals an interesting tendency that there is a great need in using various classes of Petri nets to formalize BPMN with data. this is justified by the long-existing bond between the BPMN front-end and Petri net formal backend. all such approaches also tend to offer different formalisation tasks, that is very natural given a long-standing tradition of using Petri net models for formal analysis. however, given that all such models tend to produce infinite state spaces, the authors impose boundedness on the data-related components. in our work we try to study what happens if such bounds are not introduced or what are the weaker bounds that could make such models infinite-state wrt the data they use?}

\todo[inline]{as many approaches try to study data as business artifacts, we follow the same line and say that, in general, the data we use come from a relatively abstract object domain where we can explicitly talk about components of objects (a-la relations), provide them with unique identities (a-la primary keys) and explicitly specify dependencies between them (a-la foreign-keys)}
\todo[inline]{our formalism is directly subsumed by the class of db-nets studied before. however, verification of db-nets is a hard task and, so far, none has studied any kind of more practical verification tasks for that formalism considering only its state-boundedness restriction. as a matter of fact, there is a conjecture saying that it is possible to acquire decidability of a FO variant of $\mu$-calculus for db-nets using a reduction to another foramlism of data-centric dynamic systems, by analogy with the work done on $\nu$-Petri nets. again, in this work we depart from an existing verification technique that we consider expressive and robust enough to conduct different analytic tasks intrinsic to the BPM domain. to this end, we isolate a subclass of db-nets, called \clognets and demonstrate how it can be encoded into a formalism used behind the MCMT technique. moreover, we give an example of how one can formalize business policies such as data-aware soundness on top of such nets as properties and how such properties are getting directly translated into the MCMT language.}
\todo[inline]{for this work we're going to use a setting of \mcmt working for data-aware processes called MCMT for Data-driven Applications}
Now we show how to translate a bounded \clognet $\marked{N}{m_0}$ with a fixed bound $b\in\naturals$, where $N=(\types, \schema_\types, \places,\transitions,\inflow,\outflow,\coloring,\quass,\guass)$,  into a corresponding \mcmt specification. The translation process is going to be split into two phases. First, we walk one through the representation of the type domain and catalog in \mcmt. Note that all the data components of our formalism as well as the query language were intended to have a design allowing for their seamless representation in \mcmt.
Second, we demonstrate a step-wise process of encoding of the \clognet transition enablement using array-based systems. To this end, we show on a single transition how to generate bindings based on the net marking and the content of the catalog provided by the view place queries. Finally, we encode the transition firing and new marking generation based on the acquired bindings. 




\textbf{Data types and schema translation.} All the data types from $\types=\set{\type_1,\ldots,\type_n}$ have to be represented as  corresponding sorts in \mcmt. This is done using the following declaration:
\begin{mc}
:smt (define_type D1)
...
:smt (defie_type Dn)
\end{mc}
Moreover, all the datatypes should appear in the 

We recall that \mcmt supports user-defined sorts as well as user-defined operations. However, in this paper we only consider the former and assume that every type has an equality operation defined for it. For more details on user defined operations please refer to the \mcmt documentation. \todo{cite the documentation and, if needed, remove this paragraph}

To represent the catalog relations of $\schema_\types$ in \mcmt, we need to follow the next steps. Recall that in catalog every relation schema has $n+1$ typed attributes among which some may be foreign keys referencing other relations, its first attribute is a primary key, and, finally, primary keys of different relation schemas have different types. Having these conditions in mind, we adopt a functional characterization of read-only databases studied in \cite{CGGMR19} for specifying relations in the catalog. 
For every relation $R(id,A_1,\ldots,A_n)$, where $\PK{R}=\set{id}$, we introduce unary functions that correctly reference each attribute of $R$ using its primary key. More specifically, for every $A_i$ ($i=1,\ldots,n$) we create a function $f_{R,A_i}:\dom_{\vartype(id)}\rightarrow\dom_{\vartype{A_i}}$. If $A_i$ is referencing an identifier of some other relation $S$ (i.e., $\FK{R}{A_i}{S}{id}$), then $f_{R,A_i}$ represents the foreign key referencing to $S$. Note that in this types of $A_i$ and $id$ should coincide. In \mcmt, assuming that $\texttt{id\_D}=\vartype(id)$ and $\texttt{A\_i\_D}=\vartype(A_i)$, this is going to look as follows:
\begin{mc}
:smt (define R_A_i ::(-> id_D A_i_D))
\end{mc}

%We also introduce a condition that would allow us to check whether a tuple $(x_0,\ldots,x_n)$ belongs to a relation $R$ with key dependencies on attributes $A_1$,\ldots,$A_n$:
%\[R(x_0,\ldots,x_n) \text{\,iff\,} x_0 \neq\nullv \land x_1 =f_{R,A_1}(x_0)\land \ldots\land x_n =f_{R,A_n}(x_0)\]

%\todo[inline]{do we treat sorts abstractly or shall we use more concrete sorts? (e.g., cartesian product)} 
The last missing bit are the constants that are used in the guards or arc inscriptions. They have to be explicitly defined using the following declaration:

At the end, all the aforementioned declarations have to be repeated in a special declaration used by \mcmt in the database-driven mode:
\begin{mc}
:db_driven
:db_sorts D1, ... , Dn
:db_functions  
:db_constants 
\end{mc}

\textbf{Places.} Given that every control place  along the net run is going to store at most $b$ tokens, we do not need to ensure a potentially infinite provision of values to $p$ using unbounded arrays and thus can simply use boundedly many variables. More specifically, for every place $p\in\cplaces$ with $\coloring(p)=\type_1\times\ldots\times\type_k$, we are going to introduce a $b\times k$ ``matrix'' of variables such that every row potentially stores values for each of $k$ components of some token in $p$.  In \mcmt, such variables are declared as global arrays:
\begin{mc}
:global p_11 D1
...
:global p_1k Dk
:global p_21 D1
...
:global p_bk Dk
\end{mc} 
Then, intuitively, a $j$-th token $(v_1,\ldots,v_k)\in m(p)$, where $0\leq j \leq b$, can be seen a conjunction of equalities $p_j1=v_1,\land\ldots\land\,p_jk=v_k$. Using this intuition and assuming that , we are going to represent the initial marking $m_0$ with the following special \mcmt initialization statement:

\begin{mc}
:initial
:var
:cnj $mp_1$ ... $mp_n$
\end{mc}
Here, \texttt{cnj} represents a conjunction of atomic equations that, for ease of reading, we organized in blocks, where each $mp_i$ encodes $m_0(p_i)$, for $p_i\in\cplaces$ with $\coloring(p_i)=D_1\times\ldots\times D_k$. Given that the amount of tokens in every places is bounded, we shall initialize every raw in the matrix of variables of every place by using either values of the tokens or special NULL constants. 
Now, if $m_0(p_i)\neq\mult\emptyset$, then a $j$-th token $(v_1,\ldots,v_k)\in m_0(p_i)$ is going to be represented in $mp_i$ using the following conjunction:  
\begin{mc}
(= pi_j1 v_1)(= pi_j2 v_2)...(= pi_jk v_k) 
\end{mc}
If $p_i$ has no tokens or $|m_0(p_i)|<b$, then all the related place variable are instantiated using NULL constants of the respective type. More specifically, the initialization statement for missing tokens is composed of the following conjunction:
\begin{mc}
(= pi_j1 NULL_D1)(= pi_j2 NULL_D2)...(= pi_jk NULL_Dk) 
\end{mc}




The tool adds by itself a further constant NULL S for all the above listed sorts S,


Here, \texttt{p\_i\_j} represents a $j$-th component of $p_i$. 





if a place has tokens, then every token is represented in the initialization statement using the following conjunction


if a place has no tokens or the amount of tokens is less then $b$, then every the rest of the place variables are instantiated using NULL constants of the respective type. 


We call an \emph{extended query} a query $Q$ in which every relation has been substituted with its array-based counterpart. More specifically, every relation $R(x_1,\ldots,x_n)$ from $Q$ is going to be substituted with a conjunction

\textbf{Transition enablement.}


\textbf{Places} for every place $p\in\places$ with color $\coloring(p)$  we introduce Index Sort : $p$. One can see places as schemas of the database and, thus, these elements should get 



we need to have a set of colors --> each color is a sort --> places are defined as local elements 
                         
\endinput
In case of unbounded nets, we need to represent places using arrays. To this end, every place every place $p\in\cplaces$ with $\coloring(p)=\type_1\times\ldots\times\type_k$ is going to be represented as a combination of arrays $p_1,\ldots,p_k$, where a special index type $\typename{P_{ind}}$ with domain $\dom_{P_{ind}}$ is used as the array index sort and $\type_1,\ldots,\type_k$ account for the respective target sorts of the aforementioned arrays. In \mcmt this is provided by the following declaration:
\begin{mc}
:local $p_1$ $D_1$
$\ldots$
:local $p_k$ $D_k$
\end{mc} 
Then, intuitively, given $(v_1,\ldots,v_k)\in m(p)$, we associate to it an element $e\in\dom_{P_{ind}}$ and a tuple $(e,p_1[e],\ldots,p_k[e])$, where $p_1[e]=v_1,\ldots, p_k[e]=v_k$. Here, $e$ is an internal identifier of this tuple  in $m(p)$.

to get a $e$'th token in a place $p$, one needs to write 
\textbf{What about the index sort? It has to coincide with the one from the read-only DB --> thus all the place colors should contain IDs!}

==> decidabilityMAS.tex <==
%!TEX root = main.tex



\subsection{Soundness, Completeness, Decidability}
\label{sec:theorems}

The algorithm described in Figure~\ref{fig:algorithm} describes the \emph{SMT-based backward reachability procedure} (or,
\defterm{backward search}) for handling the safety problem for an \ABMAS $\ABM$.  An integral
part of the algorithm is to compute \textit{symbolic} preimages.
%
For that purpose,  for any $\tau(\uz,\uz')$ and $\phi(\uz)$ (where $\uz'$ are renamed copies of $\uz$),
we define $\textit{Pre}(\tau,\phi)$ as the formula
$\exists \uz'(\tau(\uz, \uz')\land \phi(\uz'))$.
%
The \emph{preimage} of the set of states described by a state formula
$\phi(\ux)$ is the set of states described by
$\textit{Pre}(\tau,\phi)$ (notice that, when $\tau=\bigvee\hat\tau$,
        then $\textit{Pre}(\tau,\phi)=\bigvee\textit{Pre}(\hat\tau,\phi)$). 
%$\textit{QE}(T^*,\phi)$ in Line~6 is a subprocedure that extends the quantifier
%elimination algorithm of $T^*$ so as to convert the preimage $\textit{Pre}(\tau,\phi)$
%of a state formula $\phi$ into a state formula (equivalent to it modulo the
%axioms of $T^*$), witnessing its \emph{regressability}: this is possible since $T^*$ eliminates from primitive
%formulae the existentially quantified variables over the basic sorts,
%whereas elimination of quantified variables over artifact sorts is not
%possible, because these variables occur as arguments of artifact
%components
Backward search computes iterated preimages of a safety formula $\phi$, % and
%applies to them the above explained quantifier elimination over basic sorts, 
until a fixpoint is reached (in that case, $\ABM$ is \emph{safe} w.r.t. $\phi$) or until a set
intersecting the initial states (i.e., satisfying $\iota$) is found (in that case, $\ABM$ is \emph{unsafe} w.r.t. $\phi$) . %\footnote{
%
%The procedure is shown in Algorithm~\ref{fig:algorithm}. 
%
\textit{Inclusion} (Line~\ref{algo:while}) and \textit{disjointness} 
(Line~\ref{algo:return1}) tests can be discharged via proof obligations to be handled by SMT solvers. %AG:dic
The fixpoint is reached when the test in Line~\ref{algo:while} returns \textit{unsat}: the preimage of the set of the current states is included in the set of states reached by the backward search so far. 
%

The procedure either does not terminate or returns a \safe/\unsafe result.  
%
Given a \MASsystem $\M$ and a safety formula $\goal$, a \safe (resp. \unsafe) result is \emph{correct} iff $\ABM$ is safe (resp. unsafe) w.r.t. $\goalab$. 
%
%In what follows, we preserve the SMT terminology. \ale{non so se sia una smt terminology}

%\begin{figure}[]
%%  \begin{center}
%%  \begin{tabular}{ccc}
%%   \begin{minipage}{.15\textwidth}
%     \begin{tabular}{ll}
%       % foo \= foo \= \kill
%        \textbf{function} $\textit{BReach}(v(\ux))$ \\
%        1  $\phi\longleftarrow \psi$;  $B\longleftarrow \bot$; \\
%        2 \textbf{while} ($\phi\land \neg B$ is $T$-satisfiable) \textbf{do}\\
%        3  ~~~   \textbf{if} ($\iota\land \phi$ is $T$-satisfiable.) \\
%           ~~~   \hspace{.75cm} \textbf{then return}  $\unsafe$;\\
%        4  ~~~   $B\longleftarrow \phi\vee B$; \\
%        5  ~~~   $\phi\longleftarrow Pre(\tau, \phi);$ \\
%       % 6  ~~~   $\phi\longleftarrow \textit{QE}(T^*,\phi);$ \\
%       6 \textbf{end} \\
%        7 \textbf{return} $(\safe, B);$
%      \end{tabular}
% %   \end{minipage}
%%
%%  \end{tabular}
%%  \end{center}
%  \caption{\label{fig:algorithm}%
%    The backward reachability algorithm}
%\end{figure}





\begin{definition}
Given $\ABM$ and $\goalab$, the backward search is: 
\begin{compactitem}
\item \defterm{sound} if, when it terminates, it returns a correct result;
\item \defterm{partially sound} if a \safe result is always correct;
\item \defterm{complete} (w.r.t. detecting unsafety) if, whenever \unsafe is the correct result, then \unsafe is indeed returned.
\end{compactitem}
\label{def:properties}
\end{definition}

If partially sound, an \unsafe result may be not correct due to ``spurious''  traces. 
%
Also, as the preimage computation can diverge on a safe system, %without finding a fixpoint, 
there is no guarantee of termination.  
%Concerning \MASsystem{s} with synchronous execution semantics as in Section~\ref{sec:synchronous}, (full) soundness cannot be guaranteed, since spurious unsafe traces can be found by the backward search in case of an \unsafe result. 
%
However, since \ABMAS are a special case of the abstract \ABMAS (Def.~\ref{def:abstract-ABMAS}), we can adapt known results on array-based systems (see \cite{lmcs,CGGMR19}). 

\begin{theorem}\label{thm:sound-only}
Backward search for the safety problem is \emph{partially sound} and \emph{complete} %for handling the safety problem 
for \emph{\sync} \ABMAS. 
\end{theorem}


%For an \async \MASsystem (thus $\ABM$ as in Sec.~\ref{sec:encoding_async}):

\begin{theorem}\label{thm:sound-complete}
Backward search for the safety problem is \emph{sound} and \emph{complete} %for handling the safety problem 
for \emph{\async} \ABMAS.
\end{theorem}

It follows that, given Theorem~\ref{thm:reachable_iff_unsafe}, \myi for \sync \MASsystem we have partial soundness due to the need of using universal quantification in transition formulae (see Sec.~\ref{sec:encoding_sync}), and \myii for \async \MASsystem we have full soundness since only existential quantification is needed (see Sec.~\ref{sec:encoding_async}). 
%t
Backward search for \async \ABMAS is thus a \emph{semi-decision} procedure. %, as termination is not guaranteed. %Termination would give us a  procedure.  %\ale{dire qui 'complete' e ambiguo, perche nel teorema diciamo appunto che e 'complete', quindi dire 'give us a \emph{decision} procedure'}%If termination could be guaranteed, it would then be a complete decision procedure for (un)safety. This is the objective of the next section. 
%To this aim, we study additional conditions on the \ABMAS to guarantee termination of backward search, then becoming a full decision procedure for (un)safety.
%
Universal quantification proves to be crucial, as available results on verification of array-based systems \cite{lmcs,CGGMR19} cannot guarantee that in fact \emph{all} indexes are considered, leading to executions in which some indexes will be simply ``disregarded'' from that point on. 
%
This induces \emph{spurious} runs in the encoded \MASsystem, akin to a \emph{lossy} system \cite{lossy}. 
%, for which an analogous result is known \cite{a}. 
%



\begin{algorithm2e}[t]
\footnotesize
\SetAlgoNoEnd
\caption{backward search $\textit{BReach}(\ABM,\phi)$}
\label{fig:algorithm}
%\DontPrintSemicolon
%\SetKwFunction{analyzeConstraintGraph}{analyzeConstraintGraph}
	%\uIf{$aa$} {
	%	
	%}
	%$\phi\longleftarrow \goalab$;  
	$B\longleftarrow \bot$; \\
	\While{$\phi\land \neg B$ is \emph{satisfiable}\label{algo:while}}{
		\textbf{if} ($\iota\land \phi$ is satisfiable) \textbf{then return}  $\unsafe$\label{algo:return1};\\
		$B\longleftarrow \phi\vee B$;  $\phi\longleftarrow Pre(\tau, \phi);$ \\
	}
\KwRet  $\safe;$
\end{algorithm2e}


\subsection{A Condition for Termination}

%By exploiting the encoding from dabs to array-based artifact systems, and the soundness and completeness of backward reachability, we derive that 
%checking safety for the class of dabs satisfying these conditions is decidable.
 
We show under which (sufficient) condition we can guarantee termination of the backward search, which will gives us a decision procedure for unsafety. 
%
%While the conditions required by the technical proofs are quite
%difficult to grasp at the syntactic level, they can be intuitively understood
%using the following \emph{locality principle}: % to ensure termination,
%whenever the progression of the \MASsystem depends on the existence of some agent satisfying some guards, it does so only
%via a single agent ID in one of its templates. Hence, direct/indirect comparisons
%and joins of distinct state variables for different agent IDs within the same or different templates
%cannot be used. 
%
Although technical proofs are quite
involved at the syntactic level, they can be intuitively understood
as based on this \emph{locality condition}: the states ``visited" by the backward search can be represented by state-formulae which do not include direct/indirect comparisons and ``joins" of distinct state variables for different agent \id{s}. %, within the same or different templates. 
%
E.g., we cannot have $x^{[j_1]}=y^{[j_2]}$, which equates the current variable $x$ and $y$ of the concrete agents with \id{s} $j_1$ and $j_2$. We  can however write  $x^{[j_1]}=c$, $y^{[j_2]}=c$ for a constant $c$. 

Of course, if this property is true for $\phi$, it does not necessary hold for the formula obtained by ``regressing" $\phi$ w.r.t. some transition formula $\hat{\tau}$, i.e., $\textit{Pre}(\hat\tau,\phi)$ as those in Section~\ref{sec:mas-abs}:  $\hat\tau$ includes translations $\overline{P_t}(\act)$ of template protocols $P_t(\act)$ for action $\act$.   
%
%Therefore, it turns out that the locality condition (in our specific encoding) depends on the guards of actions in each of the agent templates of the \MASsystem which is encoded by the \ABMAS.  
%
Formally, we call a state formula \defterm{local} if it is a disjunction of the formulae of the form:
\begin{equation}\label{eq:local}
  \textstyle
  \exists j_1\cdots \exists j_m\, ( Eq(j_1,\dots, j_m)  \land
    \bigwedge_{k=1}^m \phi_k(j_k,\ux,\ua))
\end{equation}
%
Here, $Eq$ is a conjunction of
variable (dis)equalities, $\phi_k$ are quantifier-free formulae, and
$j_1,\ldots,j_m$ are individual variables of index sort. 
%
Note how 
%The key expressivity limitation of local state formulae is that they cannot
%``compare'' literals involving different agent \id{s}: in fact,
each $\phi_k$ in~\eqref{eq:local} can contain only
the existentially quantified index variable $j_k$. 
%
As said before, this limitation necessarily has an impact on transition formulae as well. We say that a transition formula $\hat\tau$ is \emph{local} 
if whenever a formula $\phi$ is local, so is
$\textit{Pre}(\hat\tau,\phi)$. 

%\begin{thm}\label{thm:decid-local}
%Backward search \emph{terminates} when applied to solve the safety problem, with respect to a \emph{ local} safety formula, for an \emph{asynchronous} \ABMAS $\M$ whose $\tau$ is a disjunction of \emph{local} transition formulae.
%\end{thm}
\begin{theorem}\label{thm:decid-local}
$\textit{BReach}(\ABM,\goalab)$ always \emph{terminates} if \myi the \ABMAS is \async and \myii its transition  formula $\tau=\bigvee\hat\tau$ is a disjunction of \emph{local} transition formulae and \myiii $\goalab$ is local.
\end{theorem}

\begin{proof}[Proof Sketch]
Although involved, the proof follows a similar argument to that of Thm.~6.2 in~\cite{CGGMR19}: 
%(a complete proof is available in~\cite{MSCS19}): 
it can be proved that an \ABMAS corresponds to a particular case of acyclic local RASs, therein defined, without ``data'',  extended with uninterpreted relations.  
\end{proof}

The locality condition is `semantic' for transition formulae and syntactic for state formulae. However, since updates in our \ABMAS by transition formulae are in fact simple assignment to constants (this can be verified by inspecting Section~\ref{sec:mas-abs}), it is immediate that, if all protocols $P_t(\act)$ are local, then $\tau$ in the \ABMAS is local.   
%A proof is here not required, since . 

\begin{example}\emph{(cont.d)} Agent protocols in our scenario satisfy locality. If modeled as an \async \MASsystem, the task is decidable.%(\async \ABMAS).
\end{example}




